Some arithmetic and geometric aspects of algebraic cycles and motives

This is my habilitation thesis. As the tradition wants, I tried to give an introduction of my field of research. I post it on the ArXiv with the hope it can be useful to young researchers looking for a short and friendly text on cohomologies of algebraic varieties, periods, algebraic cycles and motives. I might one day find the energy to expand these notes and maybe translate them in English. In the meantime, please feel free to ask questions. The first sections of this text propose an introduction to the theory, I tried to present points of view and examples which are not always stressed in the literature. A leitmotif of the thesis is the difference between phenomena in characteristic zero and those in positive characteristic. The main results are: the standard conjecture of Hodge type for abelian foufolds; the construction of a class of $p$-adic periods controlled by motivic Galois groups and for which it is possible to formulate a $p$-adic analog of the Grothendieck period conjecture; the standard conjecture of Lefschetz type for the Laza--Sacc\`a--Voisin varieties and the Chow-K\"unneth conjecture for commutative group schemes. The techniques are based on $p$-adic Hodge theory, representation theory, perverse sheaves and motivic complexes \`a la Voevodsky.

==> mynewcommands.tex <==
% personal remarks
%\newif\ifpersonal%put this line in the document
\ifpersonal
\newcommand*{\personal}[1]{\textcolor[rgb]{.2,.2,1}{\tiny{(Personal: #1)}}}
\newcommand*{\todo}[1]{\textcolor{red}{(Todo: #1)}}
\else
\newcommand*{\personal}[1]{\ignorespaces}
\newcommand*{\todo}[1]{\ignorespaces}
\fi


%%%%%code to have open/closed immersions %%%%%%%
\usetikzlibrary{decorations.markings}

\makeatletter
\tikzcdset{
	open/.code     = {\tikzcdset{hook, circled};},
	closed/.code   = {\tikzcdset{hook, slashed};},
	open'/.code    = {\tikzcdset{hook', circled};},
	closed'/.code  = {\tikzcdset{hook', slashed};},
	circled/.code  = {\tikzcdset{markwith = {\draw (0,0) circle (.375ex);}};},
	slashed/.code  = {\tikzcdset{markwith = {\draw[-] (-.0ex,-.4ex) -- (.0ex,.4ex);}};},
	markwith/.code ={
		\pgfutil@ifundefined%
		{tikz@library@decorations.markings@loaded}%
		{\pgfutil@packageerror{tikz-cd}{You need to say %
				\string\usetikzlibrary{decorations.markings} to use arrows with markings}{}}{}%
		\pgfkeysalso{/tikz/postaction = {
				/tikz/decorate,
				/tikz/decoration={markings, mark = at position 0.5 with {#1}}}
		}
	},
}
\makeatother
%%%%%%%%%%%%

\newcommand{\rB}{\mathrm B}
\newcommand{\rD}{\mathrm D}
\newcommand{\rH}{\mathrm H}
\newcommand{\rR}{\mathrm{R}}
\newcommand{\rL}{\mathrm L}
\newcommand{\rI}{\mathrm I}
\newcommand{\rb}{\mathrm b}
\newcommand{\rd}{\mathrm d}
\newcommand{\rs}{\mathrm s}
\newcommand{\rt}{\mathrm t}


\newcommand{\fA}{\mathfrak A}
\newcommand{\fB}{\mathfrak B}
\newcommand{\fC}{\mathfrak C}
\newcommand{\fD}{\mathfrak D}
\newcommand{\fH}{\mathfrak H}
\newcommand{\fS}{\mathfrak S}
\newcommand{\fT}{\mathfrak T}
\newcommand{\fU}{\mathfrak U}
\newcommand{\fV}{\mathfrak V}
\newcommand{\fX}{\mathfrak X}
\newcommand{\fY}{\mathfrak Y}
\newcommand{\fZ}{\mathfrak Z}
\newcommand{\ff}{\mathfrak f}
\newcommand{\fm}{\mathfrak m}
\newcommand{\fn}{\mathfrak n}
\newcommand{\fs}{\mathfrak s}
\newcommand{\ft}{\mathfrak t}
\newcommand{\fc}{\mathfrak{c}}

\newcommand{\cA}{\mathcal A}
\newcommand{\cB}{\mathcal B}
\newcommand{\cC}{\mathcal C}
\newcommand{\cD}{\mathcal D}
\newcommand{\cE}{\mathcal E}
\newcommand{\cF}{\mathcal F}
\newcommand{\cH}{\mathcal H}
\newcommand{\cG}{\mathcal G}
\newcommand{\cI}{\mathcal I}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cK}{\mathcal K}
\newcommand{\cL}{\mathcal L}
\newcommand{\cM}{\mathcal M}
\newcommand{\cN}{\mathcal N}
\newcommand{\cO}{\mathcal O}
\newcommand{\cP}{\mathcal P}
\newcommand{\cR}{\mathcal R}
\newcommand{\cS}{\mathcal S}
\newcommand{\cT}{\mathcal T}
\newcommand{\cU}{\mathcal U}
\newcommand{\cV}{\mathcal V}
\newcommand{\cW}{\mathcal W}
\newcommand{\cX}{\mathcal X}
\newcommand{\cY}{\mathcal Y}
\newcommand{\cZ}{\mathcal Z}


\newcommand{\bZ}{\mathbb{Z}}							  				
\newcommand{\bN}{\mathbb{N}}							  				
\newcommand{\bK}{\mathbb{K}}							  				
\newcommand{\bP}{\mathbb{P}}						
\newcommand{\bT}{\mathbb{T}}						
\newcommand{\bA}{\mathbb{A}}						
\newcommand{\bF}{\mathbb{F}}						
\newcommand{\bB}{\mathbb{B}}						
\newcommand{\bX}{\mathbb{X}}					
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bQb}{{\overline{\bQ}}}
\newcommand{\bFb}{{\overline{\bF}}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\providecommand{\bP}{\mathbb{P}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\II}{\mathbb{I}}

\newcommand{\sC}{\mathscr C}
\newcommand{\sX}{\mathscr X}
\newcommand{\sD}{\mathscr D}
\newcommand{\sU}{\mathscr U}




\newcommand{\oDelta}{\widebar\Delta}
\newcommand{\oGamma}{\widebar\Gamma}
\newcommand{\oSigma}{\widebar\Sigma}
\newcommand{\oalpha}{\widebar\alpha}
\newcommand{\obeta}{\widebar\beta}
\newcommand{\otau}{\widebar\tau}
\newcommand{\oC}{\widebar C}
\newcommand{\oD}{\widebar D}
\newcommand{\oE}{\widebar E}
\newcommand{\oG}{\widebar G}
\newcommand{\oM}{\widebar M}
\newcommand{\oS}{\widebar S}
\newcommand{\oU}{\widebar U}
\newcommand{\oW}{\widebar W}
\newcommand{\oX}{\widebar X}
\newcommand{\oY}{\widebar Y}


\newcommand{\ok}{\widebar k}
\newcommand{\ov}{\widebar v}
\newcommand{\ox}{\widebar x}
\newcommand{\oy}{\widebar y}
\newcommand{\oz}{\widebar z}

\newcommand{\hh}{\widehat h}
\newcommand{\hf}{\widehat f}
\newcommand{\hA}{\widehat A}
\newcommand{\hB}{\widehat B}
\newcommand{\hC}{\widehat C}
\newcommand{\hE}{\widehat E}
\newcommand{\hF}{\widehat F}
\newcommand{\hI}{\widehat I}
\newcommand{\hL}{\widehat L}
\newcommand{\hU}{\widehat U}
\newcommand{\hZ}{\widehat Z}
\newcommand{\hbeta}{\widehat\beta}
\newcommand{\hGamma}{\widehat\Gamma}


\newcommand{\tw}{\widetilde w}
\newcommand{\tW}{\widetilde W}
\newcommand{\tZ}{\widetilde{Z}}
\newcommand{\tk}{\tilde k}
\newcommand{\tv}{\tilde v}
\newcommand{\tB}{\widetilde B}
\newcommand{\tD}{\widetilde D}
\newcommand{\tI}{\widetilde I}
\newcommand{\tM}{\widetilde M}
\newcommand{\tN}{\widetilde N}
\newcommand{\tP}{\widetilde P}
\newcommand{\tX}{\widetilde X}
\newcommand{\tfX}{\widetilde{\fX}}
\newcommand{\tfB}{\widetilde{\fB}}
\newcommand{\tsX}{\widetilde{\sX}}
\newcommand{\tH}{\widetilde H}
\newcommand{\tY}{\widetilde Y}
\newcommand{\tbeta}{\widetilde{\beta}}
\newcommand{\tphi}{\widetilde{\phi}}
\newcommand{\ttau}{\widetilde{\tau}}



% Special symbols
\newcommand{\bcM}{\widebar{\mathcal M}}
\newcommand{\bcC}{\widebar{\mathcal C}}
% Categories
\newcommand{\Sets}{\underline{\operatorname{Sets}}}
\newcommand{\Gpds}{\underline{\operatorname{Gpds}}}
\renewcommand{\mod}{\operatorname{mod}}
\newcommand{\Rep}{\operatorname{Rep}}
\newcommand{\Inf}{\operatorname{Inf}}

%Cohomologies, realizations
\newcommand{\rHB}{\rH_{\mathrm{Betti}}}
\newcommand{\rHdR}{\rH_{\mathrm{dR}}}
\newcommand{\rHa}{\rH_{\mathrm{alg}}}
\newcommand{\rRa}{\rR_\mathrm{alg}}
\newcommand{\rRB}{\rR_\mathrm{Betti}}
\newcommand{\rRp}{\rR_{\mathrm{alg}/\bF_p}}
%motives
\newcommand{\one}{\mathbbm{1}}
\newcommand{\Mot}{{\cM ot}}
\newcommand{\Mat}{{\cM at}}
\newcommand{\Motgr}{{\Mot(\bQb)^\textrm{gr}}}
\newcommand{\MotgrQ}{{\Mot(\bQb)_{\bQ}^\textrm{gr}}}
\newcommand{\SmVar}{\cS m\cV ar}
\newcommand{\GrVect}{\mathrm{GrVect}}
\newcommand{\Fil}{\mathrm{Fil}}
\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\obF}{{\overline{\bF}}}
\newcommand{\Motp}{{\Mot(\obF_p)}}
\newcommand{\bQp}{{\bQ_p}}
\newcommand{\bQl}{{\bQ_\ell}}
\newcommand{\obQl}{{\overline{\bQ}_\ell}}
\newcommand{\obQp}{{\overline{\bQ}_p}}
\newcommand{\obQ}{{\overline{\bQ}}}
\newcommand{\cl}{\mathsf{cl}}
\newcommand{\Triples}{\mathsf{Triples}}
\newcommand{\Motss}{\Mot(\bQb)\ssing}
\newcommand{\Motsscm}{\Mot\ssing_{\mathrm{cm}}}
\newcommand{\Motssab}{\Mot\ssing_{\mathrm{ab}}}
\newcommand{\Motcm}{\Mot_{\mathrm{cm}}}
\newcommand{\Motab}{\Mot_{\mathrm{ab}}}
\newcommand{\Motm}{\Mot M} %%very temporary

\newcommand{\ssing}{^\mathrm{ss}}
\newcommand{\NUM}{\mathrm{NUM}}
\newcommand{\op}{\mathrm{op}}
\newcommand{\CHM}{\mathrm{CHM}}
\newcommand{\DM}{\mathrm{DM}}
\newcommand{\BO}{\mathrm{BO}}
\newcommand{\CM}{\mathrm{CM}}
\newcommand{\dR}{\mathrm{dR}} 
\newcommand{\crys}{\mathrm{crys}}
\newcommand{\num}{\mathrm{num}}
\newcommand{\ho}{\mathrm{hom}}
\newcommand{\mat}{\mathrm{mat}}
\newcommand{\eval}{\mathrm{eval}}

\newcommand{\Forg}{\mathsf{Forg}}

% Shorthands
\newcommand{\kc}{k^\circ}
\newcommand{\llb}{[\![}
\newcommand{\rrb}{]\!]}
\newcommand{\llp}{(\!(}
\newcommand{\rrp}{)\!)}
\newcommand{\an}{^\mathrm{an}}
\newcommand{\alg}{\mathrm{alg}}
\newcommand{\palg}{{p\text{-}\alg}}
\newcommand{\loweralg}{_\mathrm{alg}}
\newcommand{\bad}{^\mathrm{bad}}
\newcommand{\ess}{^\mathrm{ess}}
\newcommand{\ness}{^\mathrm{ness}}
\newcommand{\et}{_\mathrm{\acute{e}t}}
\newcommand{\Et}{\mathrm{\acute{E}t}}
\newcommand{\ev}{\mathsf{ev}}
% new \oset macro for overset with the symbol above lowered a bit
\makeatletter
\newcommand{\oset}[3][0.2ex]{%
	\mathrel{\mathop{#3}\limits^{
			\vbox to#1{\kern-2\ex@
				\hbox{$\scriptstyle#2$}\vss}}}}
\makeatother


\newcommand{\s}{\sigma}
\newcommand{\bs}{\bar{\sigma}}
%\providecommand{\gcd}{\mathrm{g.c.d.}}
\providecommand{\a}{\alpha}
\providecommand{\b}{\beta}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\eps}{\varepsilon}
\newcommand{\bc}{\mathsf{bc}}
\providecommand{\sst}{\mathsf{sst}}
\newcommand{\st}{\mathsf{st}}
\newcommand{\gr}{\mathsf{gr}}
\newcommand{\coZ}{{Z}^\mathrm{c}}
\newcommand{\pos}{\mathsf{pos}}
\newcommand{\reg}{\mathsf{reg}}
\newcommand{\ad}{\mathsf{ad}}
\newcommand{\pt}{\mathsf{pt}}
\newcommand{\setif}{\mathsf{setif}}
\newcommand{\acts}{\curvearrowright}

\newcommand{\inv}{^{-1}}
% Arrows
\newcommand*{\longhookrightarrow}{\ensuremath{\lhook\joinrel\relbar\joinrel\rightarrow}}
\newcommand*{\DashedArrow}[1][]{\mathbin{\tikz [baseline=-0.25ex,-latex, dashed,#1] \draw [#1] (0pt,0.5ex) -- (1.3em,0.5ex);}}

\usetikzlibrary{decorations.markings} %arrows for open immersions and closed immersions
\tikzset{
  closed/.style = {decoration = {markings, mark = at position 0.5 with { \node[transform shape, xscale = .8, yscale=.4] {/}; } }, postaction = {decorate} },
  open/.style = {decoration = {markings, mark = at position 0.5 with { \node[transform shape, scale = .7] {$\circ$}; } }, postaction = {decorate} }
}
%Reductive groups
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\GSp}{\operatorname{GSp}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\PSL}{\operatorname{PSL}}
\providecommand{\fsl}{\mathfrak{sl}}
\providecommand{\fgl}{\mathfrak{gl}}
\providecommand{\fsp}{\mathfrak{sp}}
\providecommand{\fso}{\mathfrak{so}}
\newcommand{\fg}{\mathfrak{g}}
\newcommand{\fp}{\mathfrak{p}}
\newcommand{\fu}{\mathfrak{u}}
\providecommand{\fb}{\mathfrak{b}}
\newcommand{\fh}{\mathfrak{h}}
\newcommand{\fl}{\mathfrak{l}}
\newcommand{\fk}{\mathfrak{k}}
\renewcommand\sc{\mathsf{sc}} %for simply connected
\newcommand{\Lie}{\operatorname{Lie}}

%Operators
\DeclareMathOperator{\Coker}{Coker}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\cosk}{cosk}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Frob}{Frob}
\DeclareMathOperator{\Fun}{Fun}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\cEnd}{\cE nd}
\DeclareMathOperator{\cHom}{\cH om}
\DeclareMathOperator{\Image}{Im}
\DeclareMathOperator{\Int}{Int}
\DeclareMathOperator{\Isom}{Isom}
\DeclareMathOperator{\Emb}{Emb} 
\DeclareMathOperator{\Nat}{Nat}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Map}{Map}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Jac}{{Jac}}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\RHom}{RHom}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Spf}{Spf}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\pr}{\mathsf{pr}}
\DeclareMathOperator{\jet}{\mathsf{jet}}
\DeclareMathOperator{\id}{\mathsf{id}}
\DeclareMathOperator{\Id}{\mathsf{Id}}
\DeclareMathOperator{\Ass}{\mathrm{Ass}}
\DeclareMathOperator{\Frac}{Frac}
\DeclareMathOperator{\spe}{sp}
\DeclareMathOperator{\MT}{MT}





\newcommand{\proj}{{\operatorname{proj}}}
\newcommand{\ind}{\operatorname{ind}}
\newcommand{\infl}{\operatorname{infl}}
\newcommand{\res}{\operatorname{res}}
\newcommand\can{\mathsf{can}}
\newcommand{\Ar}{\mathsf{Ar}}
\newcommand{\Betti}{\mathrm{Betti}}

\DeclareMathOperator{\tr}{trace}
\DeclareMathOperator{\trdeg}{trdeg}


% Definition of \widebar from http://tex.stackexchange.com/questions/16337/can-i-get-a-widebar-without-using-the-mathabx-package/60253#60253
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
	\setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
	\setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
	\ifdim\ht0=\ht2 #3\else #2\fi
}
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
	\begingroup
	\def\mathaccent##1##2{%
		%Enable nesting of accents:
		\let\mathaccent\save@mathaccent
		%If there's more than a single symbol, use the first character instead (see below):
		\if#32 \let\macc@nucleus\first@char \fi
		%Determine the italic correction:
		\setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
		\setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
		\dimen@\wd\tw@
		\advance\dimen@-\wd\z@
		%Now \dimen@ is the italic correction of the symbol.
		\divide\dimen@ 3
		\@tempdima\wd\tw@
		\advance\@tempdima-\scriptspace
		%Now \@tempdima is the width of the symbol.
		\divide\@tempdima 10
		\advance\dimen@-\@tempdima
		%Now \dimen@ = (italic correction / 3) - (Breite / 10)
		\ifdim\dimen@>\z@ \dimen@0pt\fi
		%The bar will be shortened in the case \dimen@<0 !
		\rel@kern{0.6}\kern-\dimen@
		\if#31
		\overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
		\advance\dimen@0.4\dimexpr\macc@kerna
		%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
		\let\final@kern#2%
		\ifdim\dimen@<\z@ \let\final@kern1\fi
		\if\final@kern1 \kern-\dimen@\fi
		\else
		\overline{\rel@kern{-0.6}\kern\dimen@#1}%
		\fi
	}%
	\macc@depth\@ne
	\let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
	zen@everymath{\mathgroup\macc@group\relax}%
	\macc@set@skewchar\relax
	\let\mathaccentV\macc@nested@a
	%The following initialises \macc@kerna and calls \mathaccent:
	\if#31
	\macc@nested@a\relax111{#1}%
	\else
	%If the argument consists of more than one symbol, and if the first token is
	%a letter, use that letter for the computations:
	\def\gobble@till@marker##1\endmarker{}%
	\futurelet\first@char\gobble@till@marker#1\endmarker
	\ifcat\noexpand\first@char A\else
	\def\first@char{}%
	\fi
	\macc@nested@a\relax111{\first@char}%
	\fi
	\endgroup
}
\makeatother




